Effective Rank Analysis and Regularization for Enhanced 3D Gaussian Splatting

3D reconstruction from multi-view images is one of the fundamental challenges in computer vision and graphics. Recently, 3D Gaussian Splatting (3DGS) has emerged as a promising technique capable of real-time rendering with high-quality 3D reconstruction. This method utilizes 3D Gaussian representation and tile-based splatting techniques, bypassing the expensive neural field querying. Despite its potential, 3DGS encounters challenges such as needle-like artifacts, suboptimal geometries, and inaccurate normals caused by the Gaussians converging into anisotropic shapes with one dominant variance. We propose using the effective rank analysis to examine the shape statistics of 3D Gaussian primitives, and identify the Gaussians indeed converge into needle-like shapes with the effective rank 1. To address this, we introduce the effective rank as a regularization, which constrains the structure of the Gaussians. Our new regularization method enhances normal and geometry reconstruction while reducing needle-like artifacts. The approach can be integrated as an add-on module to other 3DGS variants, improving their quality without compromising visual fidelity. The project page is available at https://junhahyung.github.io/erankgs.github.io.

==> tables/_dtu_results.tex <==
%\setlength\tabcolsep{0.5em}
\begin{table*}[t]
\centering
\caption{\textbf{s}}
%Quantitative comparison on the DTU Dataset~\cite{jensen2014large}}. We show the Chamfer distance and average optimization time. Our method achieves the highest reconstruction accuracy among other explicit methods.

\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{1.2mm}
\begin{tabular}{@{}llcccccccccccccccclc}
\hline \\[2pt]
 \multicolumn{3}{c}{} & 24 & 37 & 40 & 55 & 63 & 65 & 69 & 83 & 97 & 105 & 106 & 110 & 114 & 118 & 122 & & Mean  \\[4pt] \cline{4-18} \cline{19-20} \\

%\cline{4-18} \cline{20-21}

&  3DGS~\cite{kerbl3Dgaussians} & & 2.14 & 1.53 & 2.08 & 1.68 & 3.49 & 2.21 & 1.43 & 2.07 & 2.22 & 1.75 &  1.79 & 2.55 & 1.53 & 1.52 & 1.50 & & 1.96  \\
&  3DGS + Ours &  & 0.85 &  &  &  &  &  &  &  &  &  &   &  &  &  &  & &   \\ [10pt]
 &  SuGaR~\cite{guedon2023sugar} & & 1.47 & 1.33 & 1.13 & 0.61 & 2.25 & 1.71 & 1.15 & 1.63 & 1.62 & 1.07 & 0.79 & 2.45 & 0.98 & 0.88 & 0.79 & & 1.33  \\
 &  SuGaR + Ours &  &  &  &  &  &  &  &  &  &  &  &   &  &  &  &  & &   \\ [10pt]

 & 2DGS~\cite{Huang2024ARXIV} &&  \sbest 0.48 &  \tbest0.91 &  \tbest 0.39 &  \tbest 0.39 &  \sbest 1.01 &  0.83 &  0.81 &  1.36 &  1.27 &  0.76  &  0.70 &  1.40 &   \tbest 0.40 &   0.76 &  \tbest 0.52 &&  \tbest 0.80 &   \\
  &  2DGS + Ours &  &  &  &  &  &  &  &  &  &  &  &   &  &  &  &  & &   \\ [10pt]
 & GOF & & \tbest 0.50 & \sbest 0.82 & \sbest 0.37 & \sbest 0.37 & 1.12 &  0.74 & 0.73 & \sbest 1.18 & 1.29 & \best 0.68 & 0.77 & \sbest 0.90 & 0.42 & 0.66 & \sbest 0.49 && \sbest 0.74 \\
   &  GOF + Ours &  &  &  &  &  &  &  &  &  &  &  &   &  &  &  &  & &   \\ [10pt]
 \hline
\end{tabular}
}
\label{tab:dtu_result}
\end{table*}

==> tables/dtu_psnr_2.tex <==
\begin{table}
    %\vspace{-5cm}
  %\caption{Additional ablation on DTU dataset, reporting PSNR for each scene.}
  \label{tab:dtu_psnr_2}
  \centering
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
Method  & 97 & 105 & 106 & 110 & 114 & 118 & 122 & Mean \\
	
	\midrule
 3DGS & 30.20 & 34.32 & 35.00 & 34.65 & 30.86 & 37.25 & 38.07 &32.82\\
 +a & 30.25&34.30&35.11&34.59&31.10&37.65&38.21 & 32.97\\
+a+b  & 30.27& 34.41 & 35.22 & 34.69 & 31.20 & 37.69 & 38.23 &33.09\\

    \bottomrule
  \end{tabular}
  }
\end{table}

